CausalARC: Abstract Reasoning with Causal World Models

On-the-fly reasoning often requires adaptation to novel problems under limited data and distribution shift. This work introduces CausalARC: an experimental testbed for AI reasoning in low-data and out-of-distribution regimes, modeled after the Abstraction and Reasoning Corpus (ARC). Each CausalARC reasoning task is sampled from a fully specified causal world model, formally expressed as a structural causal model. Principled data augmentations provide observational, interventional, and counterfactual feedback about the world model in the form of few-shot, in-context learning demonstrations. As a proof-of-concept, we illustrate the use of CausalARC for four language model evaluation settings: (1) abstract reasoning with test-time training, (2) counterfactual reasoning with in-context learning, (3) program synthesis, and (4) causal discovery with logical reasoning. Within- and between-model performance varied heavily across tasks, indicating room for significant improvement in language model reasoning.

==> figures/demo/figure_demo.tex <==
\begin{figure}[!t]
    \centering

\begin{tikzpicture}

% SCM.
\node[draw,CornflowerBlue,rounded corners,fill=CornflowerBlue!10] (scm) at (0,0) {\begin{tabular}{l}
    \scriptsize
      \texttt{def scm():} \\
      \scriptsize
      \quad\texttt{u = np.random...} \\
      \scriptsize
      \quad\texttt{x = 6 $\cdot$ u} \\
      \scriptsize
      \quad\texttt{y = ...} 
\end{tabular}};

% L1 sample.
\node[draw,CornflowerBlue,rounded corners,fill=CornflowerBlue!10] (x) at (3.5,0) {\includegraphics[width=1cm,height=1cm]{figures/demo/x.png} $\to$ \includegraphics[width=1cm,height=1cm]{figures/demo/y.png}};
%\node[] (y) at (4.5,0) {\includegraphics[width=1cm,height=1cm]{figures/demo/y.png}};
%\draw[->,thick] (x) edge[bend left=50] (y); 

% Stack counterfactuals.
\foreach \X [count=\Z]in {3,2,1}
 {\node[opacity=1,draw,CornflowerBlue,rounded corners,fill=CornflowerBlue!10] at (8,0.75,\Z) {\includegraphics[width=1cm,height=1cm]{figures/demo/x_cf_\X.png} $\to \includegraphics[width=1cm,height=1cm]{figures/demo/y_cf_\X.png}$};}
%%
%\node[] (to) at (7.5,1.1) {};
%\node[] (from) at (5.5,1.1) {};
%\draw[->,thick] (from) edge[bend left=50] (to); 
%%
% \foreach \X [count=\Z]in {3,2,1}
% {\node[opacity=1] at (9,0.5,\Z) {\includegraphics[width=1cm,height=1cm]{figures/demo/y_cf_\X.png}};}

% Prompt.
\node[draw,CornflowerBlue,rounded corners,fill=CornflowerBlue!10] (scm) at (11.4,0) {\begin{tabular}{l}
    \scriptsize
      \texttt{You must solve the} \\
      \scriptsize
      \texttt{following puzzle by} \\
      \scriptsize
      \texttt{discovering the }\\
      \scriptsize
      \texttt{deterministic rule...}\\
      %\scriptsize
      %\texttt{maps inputs to outputs...} 
\end{tabular}};

% Labels.
\node[] (scm_label) at (0,-1.5) {\textsc{\large\textbf{a.} scm} $\mathcal{M}$};

\node[] (l1_label) at (3.5,-1.5) {{\large\textsc{\textbf{b.}}}  $(\mathbf{x}, \mathbf{y}) \sim \mathcal{M}$};

\node[] (l3_label) at (7.25,-1.5) {{\large\textsc{\textbf{c.}}}  $(\mathbf{x}', \mathbf{y}') \sim \mathcal{M}'$};

\node[] (prompt_label) at (11.4,-1.5) {\textsc{\large\textbf{d.} prompt}};



\end{tikzpicture}

    
    \caption{CausalARC testbed. \jm{Under construction: This figure is just a very rough placeholder; we need a charismatic figure here that advertises what CausalARC can be used for.}}
    \label{fig:demo}
\end{figure}

==> figures/figure_cf_reasoning_wrap.tex <==
\begin{wrapfigure}[23]{r}{0.5\linewidth}
    \centering
    %\vspace{-12mm}
    \includegraphics[width=\linewidth]{figures/logical_eval_and_xor_compose.jpg}
    \caption{Counterfactual reasoning accuracy on task \texttt{SCMtcbq} by output size.}
    \label{fig:logical_compose}
\end{wrapfigure}

==> figures/figure_motivation.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/logical_and/logical_and.png} \\
    \caption{In-context learning with demonstrations sampled from L1 (associational level) versus L3 (counterfactual level) of the PCH. Demonstration pairs were sampled from an SCM identical to Example \ref{example:scm_xor} where logical \textit{and} replaces logical \textit{xor}, colors are permuted, and the dimensionality of the output array scales ($3 \times 3$, $4 \times 4$, $5 \times 5$). L3 demonstrations induced better or equal performance relative to L1 demonstrations. L3 demonstrations combined with a fully specific SCM (provided in-context as a Python program) provided better or equal performance relative to L3 demonstrations alone. Metric ($1 -$ Hamming Distance) measures the proportion of array elements that are correct, with a maximum score of 1.}
    \label{fig:motivating_example}
\end{figure}

==> figures/in_text_bar_charts.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/logical_eval_and_xor_compose.jpg}
    \caption{Counterfactual reasoning by array size and prompt PCH level on logical composition task \texttt{SCMtcbq} (\textit{xor} after \textit{and}). Scores were over five random prompt samples.}
    \label{fig:logical_compose}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\linewidth]{figures/program_synthesis_bar_l1.jpg} \hspace{5mm}
    \includegraphics[width=0.4\linewidth]{figures/discovery_logical_compose_and_xor_l1.jpg}
    \caption{(Left) Program synthesis on four counting and extension tasks as total in-context demonstrations increased. (Right) Causal discovery with logical reasoning as array size increased. Scores were over five random L1 prompt samples. Results for L3 prompts are in Appendix \ref{appendix:experimental_results}}
    \label{fig:prog_synth_discovery_in_text}
\end{figure}

==> figures/pc.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/discovery/pc_and_10000.png} \\
    \includegraphics[width=\linewidth]{figures/discovery/pc_or_10000.png} \\
    \includegraphics[width=\linewidth]{figures/discovery/pc_xor_10000.png}
    \caption{Caption}
    \label{fig:placeholder}
\end{figure}

==> tables/table_discovery.tex <==
\begin{table}[!t]
    \centering
    \begin{tabular}{l c c}
    \toprule[1pt]
        & \textsc{L1 prompts} & \textsc{L3 prompts} \\
        \midrule
        \textit{Claude Haiku 3} & 0.0 & \textbf{0.4} \\
        \textit{GPT-4o mini} & 0.0 & \textbf{0.4} \\
        \textit{o4 mini} & \textbf{1.0} & 0.9 \\
        \textit{Gemini 2.5 Flash} & 0.6 & \textbf{0.9} \\
    \bottomrule[1pt]
    \end{tabular}
    \vspace{2mm}
    \caption{Correct prediction of the logical operator that acts as the causal function in CausalARC task SCMdky5. Results were out of ten replicates (5 logical \textit{or}, 5 logical \textit{and}), where replicates were unique randomly sampled task prompts. \jm{Add prompts and hyperparameters to appendix; repeat experiments with more replicates and causal functions.} Bold denotes best performance.}
    \label{tab:logical_discovery}
\end{table}

==> tables/table_discovery_old.tex <==
\begin{table}[!t]
    \centering
    \begin{tabular}{l c c c c}
    \toprule[1pt]
        & \multicolumn{2}{c}{\textsc{logical and}} & \multicolumn{2}{c}{\textsc{logical or}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & \textit{L1 prompts} & \textit{L3 prompts} & \textit{L1 prompts} & \textit{L3 prompts} \\
        \midrule
        \textit{Claude Haiku 3} & 0.0 & \underline{\textbf{0.2}} & 0.0 &  \underline{\textbf{0.6}}\\
        \textit{GPT-4o mini} & 0.0 & \underline{\textbf{0.8}} & \textbf{0.0} & \textbf{0.0 }\\
        \textit{o4 mini} & \textbf{1.0} & \textbf{1.0} & \underline{\textbf{1.0}} & 0.8 \\
        \textit{Gemini 2.5 Flash} & \textbf{1.0} & \textbf{1.0} & 0.2 & \underline{\textbf{0.8}} \\
    \bottomrule[1pt]
    \end{tabular}
    \vspace{2mm}
    \caption{Correct prediction of the logical operator that acts as the causal function in CausalARC task SCMdky5. Results were out of five replicates, where replicates were unique randomly sampled task prompts. \jm{Add prompts and hyperparameters to appendix.} Bold denotes equal or better performance, while bold underline denotes strictly better performance.}
    \label{tab:logical_discovery}
\end{table}

==> tables/table_illustrative_example.tex <==
\begin{table}[!t]
    \centering
    \begin{tabular}{l c c}
    \toprule[1pt]
        & \multicolumn{2}{c}{\textsc{Correct}} \\
        \cmidrule(lr){2-3} 
        & \textit{Without cfs} & \textit{With cfs} \\
        \midrule
        \textit{ChatGPT (GPT-5)} & \cmark & \cmark \\
        \textit{Claude Sonnet 4} & \cmark & \cmark \\
        \textit{DeepSeek Chat (V3)} & \cmark & \cmark \\
        \textit{Gemini 2.5 Flash} & \xmark & \cmark \\
        \textit{Grok 3} & \xmark & \cmark \\
    \bottomrule[1pt]
    \end{tabular}
    \caption{Caption}
    \label{tab:placeholder}
\end{table}

